Connecting the Dots between Audio and Text without Parallel Data through Visual Knowledge Transfer

Machines that can represent and describe environmental soundscapes have practical potential, e.g., for audio tagging and captioning systems. Prevailing learning paradigms have been relying on parallel audio-text data, which is, however, scarcely available on the web. We propose VIP-ANT that induces \textbf{A}udio-\textbf{T}ext alignment without using any parallel audio-text data. Our key idea is to share the image modality between bi-modal image-text representations and bi-modal image-audio representations; the image modality functions as a pivot and connects audio and text in a tri-modal embedding space implicitly. In a difficult zero-shot setting with no paired audio-text data, our model demonstrates state-of-the-art zero-shot performance on the ESC50 and US8K audio classification tasks, and even surpasses the supervised state of the art for Clotho caption retrieval (with audio queries) by 2.2\% R@1. We further investigate cases of minimal audio-text supervision, finding that, e.g., just a few hundred supervised audio-text pairs increase the zero-shot audio classification accuracy by 8\% on US8K. However, to match human parity on some zero-shot tasks, our empirical scaling experiments suggest that we would need about $2^{21} \approx 2M$ supervised audio-caption pairs. Our work opens up new avenues for learning audio-text connections with little to no parallel audio-text data.

==> figure/retrieval_clf_level_of_supervision.tex <==
\begin{figure*}[!t!]
	\centering
	\begin{subfigure}{.48\linewidth}
		\begin{center}
		\includegraphics[width=.99\linewidth]{figure/al_level_of_supervision.pdf}  
		\end{center}
		\vskip -.25em
		\caption{\label{fig:retrieval_level_of_supervision}
	R@1 of AT retrieval on AudioCaps test set.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.48\linewidth}
	\begin{center}
	\includegraphics[width=.99\linewidth]{figure/al_esc50_us8k_level_of_supervision.pdf}  
	\end{center}
	\vskip -.25em
	\caption{\label{fig:clf_level_of_supervision}
	Zero-shot classification (CLF) on ESC50 and US8K.}
	\end{subfigure}
	\vspace{-.55em}
	\caption{\label{fig:retrieval_clf_level_of_supervision}
	Audio retrieval and zero-shot classification performance versus level of language supervision.}
\end{figure*}

==> figure/trimodal_consistency.tex <==
\begin{figure*}[!t]
	\centering
	\begin{subfigure}{.48\linewidth}
		\begin{center}
		\includegraphics[width=.99\linewidth]{figure/avta.pdf}  
		\end{center}
		\vskip -.25em
		\caption{\label{fig:trimodal_consistency}
	Tri-modal consistency.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.48\linewidth}
	\begin{center}
	\includegraphics[width=.99\linewidth]{figure/avl_pivot_va_gc_rc.pdf}  
	\end{center}
	\vskip -.25em
	\caption{\label{fig:image_pivot}
	Pivoting audio and text with image.}
	\end{subfigure}
	\vspace{-.55em}
	\caption{\label{fig:trimodal_pivot} Tri-modal consistency of \modelname and the versions fine-tuned on GC and RC. The evaluation is conducted on the test set of AudioCaps.}
\end{figure*}

==> figure/zeroshot_clf_prompt.tex <==
\begin{figure*}[!t]
	\centering
	\begin{subfigure}{.32\linewidth}
		\centering
		\includegraphics[width=.99\linewidth]{figure/al_bar_esc50_prompt.pdf}  
		\vskip -.25em
		\caption{\label{fig:clf_prompt_esc50} ESC50}
	\end{subfigure}
	\begin{subfigure}{.32\linewidth}
	\centering
	\includegraphics[width=.99\linewidth]{figure/al_bar_us8k_prompt.pdf}  
	\vskip -.25em
	\caption{\label{fig:clf_prompt_us8k} US8K}
	\end{subfigure}
	\begin{subfigure}{.32\linewidth}
	\centering
	\includegraphics[width=.99\linewidth]{figure/al_bar_as_prompt.pdf} 
	\vskip -.25em
	\caption{\label{fig:clf_prompt_as} AudioSet}
	\end{subfigure}	
	\vspace{-.55em}
	\caption{\label{fig:zeroshot_clf_prompt}
		Zero-shot audio classification with / without using the prompt "the sound of". \modelname is our base model and has been pre-trained on VA data.
		We further fine-tune it on AT data, which is curated using different strategies: GL, GC, AC, FC, VC, RC (see Table~\ref{tab:al_curation} for details).}
\end{figure*}

==> table/al_curation.tex <==
\begin{table*}[!t]\small
	\centering
	{\setlength{\tabcolsep}{0.em} %{.25em}
		\makebox[\linewidth]{\resizebox{.95\linewidth}{!}{%
				\begin{tabular}{m{0.05\linewidth} @{} m{0.1\linewidth} @{\hspace{0.05cm}} m{0.85\linewidth} @{}}
				\toprule
					\multirow{16}{*}{\rotatebox[origin=c]{90}{ Unsupervised Curation}}
					& \textbf{AC}  & \textbf{A}udio-focused \textbf{C}aptions originate from the training captions of AudioCaps and Clotho. We perform caption retrieval by using CLIP and the prompt "the sound of". \\
					\cmidrule{3-3}
					&example & \textit{A balloon is rubbed quickly and slowly to make squeaking sounds.} \\
					\cmidrule{2-3}
					&\textbf{FC} & \textbf{F}ree \textbf{C}aptions are generated by priming GPT-J with MSCOCO captions. We perform caption retrieval by using CLIP and the prompt "a photo of". \\
					\cmidrule{3-3}
					&example & \textit{The blue colored person is jumping on the white and yellow beach ball.} \\					
					\cmidrule{2-3}
					&\textbf{VC} & \textbf{V}ision-focused \textbf{C}aptions originate from MSCOCO. We perform caption retrieval by using CLIP and the prompt "a photo of". \\
					\cmidrule{3-3}
					&example & \textit{A sky view looking at a large parachute in the sky.}\\
					\cmidrule{2-3}
					&\textbf{RC} & \textbf{R}andom \textbf{C}aptions indicates that we break the gold AT alignment in AudioCaps by randomly sampling a caption for each audio clip. They are used as a lower bound on the quality of AT alignment. \\
					\cmidrule{2-3}
					&example & \textit{A whoosh sound is heard loudly as a car revs its engines.} \\
					\midrule
					\multirow{4}{*}{\rotatebox[origin=c]{90}{Few-shot Curation}}&\textbf{GL} & \textbf{G}old textual \textbf{L}abels of audio clips are used to construct AT pairs. \\
					\cmidrule{3-3}
					&example & \textit{Gurgling}\\
					\cmidrule{2-3}
					&\textbf{GC} & \textbf{G}old \textbf{C}aptions from AudioCaps provide an upper bound on the quality of AT alignment. \\
					\cmidrule{3-3}
					&example & \textit{Children screaming in the background as the sound of water flowing by.} \\
					\bottomrule
	\end{tabular}}}}
	\vspace{3pt}
    \includegraphics[width=0.92\linewidth]{figure/caption_example.pdf}
    
	\caption{\label{tab:al_curation}
		Different ways of curating AT pairs. \textit{Gurgling} is described as "the bubbling sound of water flowing through a narrow constriction, such as from a bottle with a narrow neck". The example comes from this YouTube video: \href{https://youtu.be/1O7-QuhweZE?t=19}{1O7-QuhweZE}. The video clip starts at 19 seconds and lasts for 10 seconds (see video frames used for caption retrieval in Figure~\ref{fig:example_vframes}). \jack{I'm a bit concerned that the examples here for the unsupervised curation are not ``good" enough to give a sense that they are even better than random... They are quite noisy, but the examples presented here maybe don't give the reader enough of a sense that they /sometimes/ are reasonable.}
		\youngjae{how about showing the frames of 1O7-QuhweZE near the table? (like this,, need modification also) and It would be nice if it was possible to find better examples or to bring other examples of FC and AC etc. } \youngjae{and use audio visualizer and overlay tags the peak points manually,  "screaming", "gurgling" "splashing"}
	}
\end{table*}

==> table/al_curation_better_table.tex <==
\begin{table*}[t]\small
	\centering
	{\setlength{\tabcolsep}{0pt} %{.25em}
		\makebox[\linewidth]{\resizebox{1.\linewidth}{!}{%
				\begin{tabular}{@{} m{0.03\linewidth} @{\hspace{0.0cm}} m{0.08\linewidth} @{\hspace{0.0cm}} m{0.75\linewidth} @{}}
					\toprule
					\multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize Supervised}}}
					&\textbf{GL} & \textbf{G}old textual \textbf{L}abels are used to construct AL pairs. {(120816 aligned pairs)} \\
%					\cmidrule{2-2}
					&example & \coloredrow{1}{olive!5}{\textit{Gurgling}} \\
					\cmidrule{2-3}
					&\textbf{GC} & \textbf{G}old \textbf{C}aptions from AudioCaps provide an upper bound on the quality of AL alignment. {(44118 aligned pairs)} \\
%					\cmidrule{2-2}
					&example &\coloredrow{1}{olive!5}{\textit{Children screaming in the background as the sound of water flowing by.}} \\
					\cdashlinelr{1-3}
				% 	\cdashline{1-3}
				    % \hdashline
					\multirow{12}{*}{\rotatebox[origin=c]{90}{{\footnotesize Unsupervised}}}
					&\textbf{AC}  & \textbf{A}udio-focused \textbf{C}aptions originate from the training captions of AudioCaps and Clotho. We perform caption retrieval by using CLIP and the prompt "the sound of". {(1080078 aligned pairs)} \\
%					\cmidrule{2-2}
					&example & \coloredrow{1}{olive!5}{\textit{A balloon is rubbed quickly and slowly to make squeaking sounds.}} \\
					\cmidrule{2-3}
					&\textbf{FC} & \textbf{F}ree \textbf{C}aptions are generated by priming GPT-J with MSCOCO captions. We perform caption retrieval by using CLIP and the prompt "a photo of". {(1224621 aligned pairs)} \\
%					\cmidrule{2-2}
					&example & \coloredrow{1}{olive!5}{\textit{The blue colored person is jumping on the white and yellow beach ball.}} \\					
					\cmidrule{2-3}
					&\textbf{VC} & \textbf{V}ision-focused \textbf{C}aptions originate from MSCOCO. We perform caption retrieval by using CLIP and the prompt "a photo of". {(1172276 aligned pairs)}\\
%					\cmidrule{2-2}
					&example & \coloredrow{1}{olive!5}{\textit{A sky view looking at a large parachute in the sky.}}\\
					\cmidrule{2-3}
					&\textbf{RC} & \textbf{R}andom \textbf{C}aptions indicates that we break the gold AL alignment in AudioCaps by randomly sampling a caption for each audio clip. They are used as a lower bound on the quality of AL alignment. {(44118 aligned pairs)} \\
%					\cmidrule{2-2}
					&example & \coloredrow{1}{olive!5}{\textit{A whoosh sound is heard loudly as a car revs its engines.}} \\
					\bottomrule
	\end{tabular}}}}
	\centering
	{\setlength{\tabcolsep}{0pt} %{.25em}
	\makebox[\linewidth]{\resizebox{1.\linewidth}{!}{%
			\begin{tabular}{@{} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} @{\hspace{0.003\linewidth}} 
					m{0.097\linewidth} 
					@{}}
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_01.jpg}} &
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_02.jpg}} &
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_03.jpg}} &
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_04.jpg}} & \raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_05.jpg}} &
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_06.jpg}} &
	\raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_07.jpg}} & \raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_08.jpg}} &
	 \raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_09.jpg}} &
	 \raisebox{-\totalheight}{\includegraphics[width=\linewidth]{figure/1O7-QuhweZE/p0_12_10.jpg}} \\
%	 \bottomrule
	\end{tabular}}}}								
	\caption{\label{tab:al_curation}
		Different ways of curating AT pairs. \textit{Gurgling} is described as "the bubbling sound of water flowing through a narrow constriction, such as from a bottle with a narrow neck". The example comes from this YouTube video: \href{https://www.youtube.com/watch?v=1O7-QuhweZE}{1O7-QuhweZE}.
% 		\jack{yann: can you add the number of pairs?}
% 		It is a 10-second video clip and starts at 19 seconds
% 		.\jack{I'm a bit concerned that the examples here for the unsupervised curation are not ``good" enough to give a sense that they are even better than random... They are quite noisy, but the examples presented here maybe don't give the reader enough of a sense that they /sometimes/ are reasonable.}
% 		\yanpeng{they are better than random: RC does not mention children and water, but both of them present in the audio and are mentioned in GC.}
% 		\youngjae{how about showing the frames of 1O7-QuhweZE near the table? (like this,, need modification also) and It would be nice if it was possible to find better examples or to bring other examples of FC and AC etc. } \youngjae{and use audio visualizer and overlay tags the peak points manually,  "screaming", "gurgling" "splashing"}\yanpeng{what is wrong with the current FC and AC?}
	}
	\vspace{-.25em}
\end{table*}

==> table/classification.tex <==
\begin{table}[!t]
	{\setlength{\tabcolsep}{.2em}
	\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
	\begin{tabular}{
			@{} p{0.4cm} 
			@{\hspace{0.05cm}} p{2.cm} 
			@{\hspace{0.35cm}} p{1.65cm} 
			@{\hspace{0.25cm}} p{1.65cm} 
			@{\hspace{0.25cm}} p{1.55cm} 
			@{}
	}
%		&  & \multicolumn{2}{c}{\hspace{-2mm}{\scriptsize EK100 (R@5; \%) }} \\
		&  Model & ESC50 & US8K & AS \\ \toprule
		\multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize Supervised}}} 
		&  AST-S      & 88.7$_{\pm 0.7}$       &   & 31.4$^\star$ \\
		&  AST-P      & 95.6$_{\pm 0.4}$       &   &  \\
		\cmidrule{2-5}
		&  Random & 55.5$_{\pm 4.1}$ & 71.7$_{\pm 5.2}$ & \leavevmode{\phantom{0}}6.1 \\
		&  CLIP & 89.7$_{\pm 1.5}$ & 82.5$_{\pm 6.0}$ & 17.2 \\
% 		&  \modelname probe & 79.3$_{\pm 3.0}$ & 82.0$_{\pm 4.7}$ & 18.1 \\
		&  \modelname & \textbf{95.7}$_{\pm 1.4}$ & \textbf{86.0}$_{\pm 2.8}$ & \textbf{37.9} \\
% 		& +AT w/ GC & \textbf{96.3}$_{\pm 0.6}$ & 81.0$_{\pm 5.14}$ & 37.9 \\ 
		\midrule
% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/ $p$}}} 
		\multirow{3}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot}}} 
% 		&  CLIP      &  1.9   &  9.2 & 0.6 \\
% 		\cmidrule{2-5}
        &  VA-Rand & 37.6{\footnotesize (33.0)} & 41.9{\footnotesize (38.1)} & \leavevmode{\phantom{0}}1.7{\footnotesize (\phantom{0}2.0)} \\
		&  \modelname     &   57.1{\footnotesize (49.9)}   & 44.7{\footnotesize (37.8)}  &  \leavevmode{\phantom{0}}2.6{\footnotesize (\phantom{0}2.8)} \\
		\cmidrule{2-5}
% 		&  +AT w/ VC     &   61.9   &  52.7  &  \leavevmode{\phantom{0}}8.9 \\
% 		&  +AT w/ AC      &   62.8   &  54.0  &  11.6 \\
% 		&  +AT w/ FC     &  62.5    & 52.7   & 11.2 \\
		&  +AT w/ GC     &  69.2{\footnotesize (64.3)}    &  71.7{\footnotesize (67.1)}  & 13.3{\footnotesize (13.6)} \\
% 		&  +AT w/ RC     &   51.6   &  42.3  &  \leavevmode{\phantom{0}}4.1 \\
% 		&  +AT w/ GL     &   67.4   &  62.9  &  15.4 \\
% 		\midrule
% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/o $p$}}} 
% 		&  CLIP      &   2.2   &  6.1  &  0.6 \\
% 		\cmidrule{2-5}
%         &  VA-Rand     & 33.0 & 38.1 & \leavevmode{\phantom{0}}2.0 \\
% 		&  \modelname     &   49.9  &  37.8  &  \leavevmode{\phantom{0}}2.8 \\
% 		\cmidrule{2-5}
% 		&  +AT w/ VC     &   58.0   &  50.3  &  10.7 \\
% 		&  +AT w/ AC      &  55.7   &  47.0  &  12.3 \\
% 		&  +AT w/ FC     &  58.0    & 50.0   & 12.2 \\
% 		&  +AT w/ GC     &   64.3   &  67.1  &  13.6 \\
% 		&  +AT w/ RC     &   36.1   &  28.5  &  \leavevmode{\phantom{0}}4.6 \\
% 		&  +AT w/ GL     &   64.3   &  60.9  &  18.9 \\
		\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:zeroshot-clf}
		Supervised and zero-shot audio classification accuracies (\%) on ESC50 and US8K and mAPs (\%) on AS. 
		AST-S and AST-P are the state-of-the-art models from~\citet{AST}.
% 		$^\star$ indicates that we follow AST's settings and train and evaluate it on our data.
        In the supervised setting, Random, CLIP, \modelname, and "+AT w/ GC" indicate that the audio encoder is initialized randomly, from CLIP, and from \modelname, respectively.
        % from \modelname, and from \modelname+AT (fine-tuned on gold AT pairs of AudioCaps), respectively.
        In the zero-shot setting, we use a prompt "the sound of" by default; accuracies in the parenthesis are obtained without using the prompt. "+AT w/ GC" means that we fine-tune \modelname on gold AT pairs of AudioCaps.
% 		$p$ represents the prompt `the sound of'. VC, AC, FC, RC, GC indicate different caption augmentation strategies (see Section~\ref{sec:audio_text_aug} for details).
% 		and stand for \textbf{V}ision-focused, \textbf{A}udio-focused, \textbf{F}ree (generated by GPT-J), \textbf{G}old captions, and \textbf{R}andom gold captions, respectively. GL means that \textbf{G}old \textbf{L}abels of audios are used as captions.
	}
	\label{tab:ek100table}
\end{table}

==> table/classification_merged_prompt.tex <==
\begin{table}[!t]
	{\setlength{\tabcolsep}{.2em}
		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
				\begin{tabular}{
						@{} p{0.4cm}
						@{\hspace{0.05cm}} p{2.7cm} 
						@{\hspace{0.35cm}} p{1.65cm} 
						@{\hspace{0.25cm}} p{1.65cm} 
						@{\hspace{0.25cm}} p{1.55cm} 
						@{}
					}
					%		&  & \multicolumn{2}{c}{\hspace{-2mm}{\scriptsize EK100 (R@5; \%) }} \\
					&  Model & ESC50 & US8K & AS \\ \toprule
					\multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize }}} 
%					&  AST-S      & 88.7$_{\pm 0.7}$       &   & 31.4$^\star$ \\
%					&  AST-P      & 95.6$_{\pm 0.4}$       &   &  \\
%					\cmidrule{2-5}
%					&  Random & 55.5$_{\pm 4.1}$ & 71.7$_{\pm 5.2}$ & \leavevmode{\phantom{0}}6.1 \\
%					&  CLIP & 89.7$_{\pm 1.5}$ & 82.5$_{\pm 6.0}$ & 17.2 \\
					% 		&  \modelname probe & 79.3$_{\pm 3.0}$ & 82.0$_{\pm 4.7}$ & 18.1 \\
%					&  \modelname & \textbf{95.7}$_{\pm 1.4}$ & \textbf{86.0}$_{\pm 2.8}$ & \textbf{37.9} \\
					&  Supervised & \text{95.7}$_{\pm 1.4}$ & \text{86.0}$_{\pm 2.8}$ & \text{37.9} \\
					
					% 		& +AT w/ GC & \textbf{96.3}$_{\pm 0.6}$ & 81.0$_{\pm 5.14}$ & 37.9 \\ 
					\midrule
					% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/ $p$}}} 
					\cmidrule{2-5}
					\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot}}} 
					% 		&  CLIP      &  1.9   &  9.2 & 0.6 \\
					% 		\cmidrule{2-5}
					&  VA-Rand & 37.6{\footnotesize (33.0)} & 41.9{\footnotesize (38.1)} & \leavevmode{\phantom{0}}1.7{\footnotesize (\phantom{0}2.0)} \\
					&  \modelname     &   57.1{\footnotesize (49.9)}   & 44.7{\footnotesize (37.8)}  &  \leavevmode{\phantom{0}}2.6{\footnotesize (\phantom{0}2.8)} \\
					\cmidrule{2-5}
					&  +AT w/ GL     &   67.2{\footnotesize (64.5)}    &  62.6{\footnotesize (61.0)}   &  15.4{\footnotesize (\textbf{18.9})}  \\
					&  +AT w/ GC     &  \textbf{69.5}{\footnotesize (64.2)}    &  \textbf{71.9}{\footnotesize (67.1)}  & 13.3{\footnotesize (13.6)} \\
				% 	&  +AT w/ GL     &   67.4{\footnotesize (64.3)}    &  62.9{\footnotesize (60.9)}   &  15.4{\footnotesize (\textbf{18.9})}  \\
				% 	&  +AT w/ GC     &  69.2{\footnotesize (64.3)}    &  \textbf{71.7}{\footnotesize (67.1)}  & 13.3{\footnotesize (13.6)} \\
					& AudioCLIP & \text{69.4} & 65.3 &  \\
					\cdashlinelr{2-5}
	 		 		&  +AT w/ AC      &   62.8{\footnotesize (55.7)}   &  54.0{\footnotesize (47.0)}  &  11.6{\footnotesize (12.3)} \\
	 		 		&  +AT w/ FC     &  62.5{\footnotesize (58.0)}    & 52.7{\footnotesize (50.0)}   & 11.2{\footnotesize (12.2)} \\
	 		 		&  +AT w/ VC     &   61.9{\footnotesize (58.0)}   &  52.7{\footnotesize (50.3)}  &  \leavevmode{\phantom{0}}8.9{\footnotesize (10.7)} \\
	 		 		&  +AT w/ RC     &   51.6{\footnotesize (36.1)}    &  42.3{\footnotesize (28.5)}   &  \leavevmode{\phantom{0}}4.1{\footnotesize (\phantom{0}4.6)} \\
	 		 		& Wav2CLIP & 41.4 & 40.4 &  \\
					% 		\midrule
					% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/o $p$}}} 
					% 		&  CLIP      &   2.2   &  6.1  &  0.6 \\
					% 		\cmidrule{2-5}
					%         &  VA-Rand     & 33.0 & 38.1 & \leavevmode{\phantom{0}}2.0 \\
					% 		&  \modelname     &   49.9  &  37.8  &  \leavevmode{\phantom{0}}2.8 \\
					% 		\cmidrule{2-5}
%					 		&  +AT w/ VC     &   58.0   &  50.3  &  10.7 \\
%					 		&  +AT w/ AC      &  55.7   &  47.0  &  12.3 \\
%					 		&  +AT w/ FC     &  58.0    & 50.0   & 12.2 \\
%					 		&  +AT w/ GC     &   64.3   &  67.1  &  13.6 \\
%					 		&  +AT w/ RC     &   36.1   &  28.5  &  \leavevmode{\phantom{0}}4.6 \\
%					 		&  +AT w/ GL     &   64.3   &  60.9  &  18.9 \\
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:zeroshot-clf-merged-prompt}
		Zero-shot audio classification accuracies (\%) on ESC50 and US8K and mAPs (\%) on AudioSet (AS). 
%		AST-S and AST-P are the state-of-the-art models from~\citet{AST}.
		% 		$^\star$ indicates that we follow AST's settings and train and evaluate it on our data.
%		In the supervised setting, Random, CLIP, \modelname, and "+AT w/ GC" indicate that the audio encoder is initialized randomly, from CLIP, and from \modelname, respectively.
		"Supervised" indicates that we fine-tune \modelname for supervised audio classification. 
		% from \modelname, and from \modelname+AT (fine-tuned on gold AT pairs of AudioCaps), respectively.
		In the zero-shot setting, we use a prompt `\textit{the sound of}' by default; accuracies in the parenthesis are obtained without using the prompt. "+AT" means that we fine-tune \modelname on AT pairs curated through different ways.
		AudioCLIP is pre-trainined using the 2 million textual labels of AudioSet; +AT w/ GL and +AT w/ GC are trained with only 44K labels / captions. Wav2CLIP is most directly comparable to our fully unsupervised pivoting model \modelname.
% 		\jack{yann, can you check these captions?}
		% 		$p$ represents the prompt `the sound of'. VC, AC, FC, RC, GC indicate different caption augmentation strategies (see Section~\ref{sec:audio_text_aug} for details).
		% 		and stand for \textbf{V}ision-focused, \textbf{A}udio-focused, \textbf{F}ree (generated by GPT-J), \textbf{G}old captions, and \textbf{R}andom gold captions, respectively. GL means that \textbf{G}old \textbf{L}abels of audios are used as captions.
	}
	\vspace{-.25em}
\end{table}

==> table/clf_audioset.tex <==
\begin{table}[t]
	{\setlength{\tabcolsep}{.75em}
		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
				\begin{tabular}{
						@{\hspace{0.05cm}} p{1.5cm} 
						@{\hspace{0.55cm}} P{1.0cm}
						@{\hspace{0.35cm}} P{1.0cm}
						@{\hspace{0.35cm}} P{1.0cm}
						@{\hspace{0.35cm}} P{1.5cm}
				% 		@{\hspace{0.3cm}} P{1.8cm}
						%						@{}
					}
				Dataset & AST &  AST$^\star$ & AST$^\dagger$ &  \modelname \\ %& +AT w/ GC \\
				\midrule
				Unbalanced & & & 43.4 & \textbf{44.7} \\
				Balanced  & 34.7 & 35.8 & 31.4 & \textbf{37.9} \\ % & \textbf{37.9} \\
				\bottomrule 
	\end{tabular}}}}
	\caption{\label{tab:clf-audioset}
		Multi-label classification mAPs (\%) on AS.
		AST indicates the results reported by~\citet{AST}. We follow their suggestions and test the their best model (AST$^\star$) on our test set. Note that the best model has been trained on the combination of balanced and unbalanced AS training sets. $^\dagger$ indicates that we follow the settings of AST and train it on our data. 
		%"+AT w/ GC" means that \modelname is fine-tuned on gold AT pairs of AudioCaps.
	}
\end{table}

==> table/dataset_and_task.tex <==
\begin{table}[!t]\small
	\centering
	%	\setlength{\tabcolsep}{.35em}
	{\setlength{\tabcolsep}{.25em}
		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
				\begin{tabular}{rccccc}
				% 	\toprule
					{Task} & 
					\multicolumn{1}{l}{{ESC50}} & 
					\multicolumn{1}{l}{{US8K}} &
					\multicolumn{1}{l}{{AudioSet}} &
					\multicolumn{1}{l}{{AudioCaps}} &
					\multicolumn{1}{l}{{Clotho}}  \\
					\midrule
					VA retrieval &  &  & \checkmark  &\\
					AL retrieval & & & & \checkmark & \checkmark \\
					Zero-shot CLF & \checkmark & \checkmark  & \checkmark & \\
					Supervised CLF & \checkmark & \checkmark & \checkmark & \\
					Audio captioning & & & & \checkmark & \checkmark \\ 
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:data_and_task}
		Datasets and tasks considered in this work (see Table~\ref{tab:data_stats} in Appendix~\ref{app:data_stats} for data statistics). CLF stands for 'classification'.
	}
	\vspace{-.1em}
\end{table}

==> table/hyperparam_va_al_esc50_us8k.tex <==
\begin{table}[t]\small
	\centering
	{\setlength{\tabcolsep}{0.em} %{.25em}
		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
				\begin{tabular}{
						@{} m{0.01\linewidth} 
						@{} m{0.30\linewidth} 
						@{\hspace{0.25cm}} M{0.125\linewidth} 
						@{\hspace{0.25cm}} M{0.125\linewidth} 
						@{\hspace{0.25cm}} M{0.125\linewidth} 
						@{\hspace{0.25cm}} M{0.125\linewidth} 
%						@{}
					}
					\toprule
%					\multirow{7}{*}{\rotatebox[origin=c]{90}{{\footnotesize VA Pre-training}}} 
					& Hyperparam. & VA & AT & ESC50 & US8K \\
					\midrule
					& Optimizer & \bothmodels{4}{LARS~\citep{LARS}}{olive!5}\\ 
					& Batch size & 432 & 64 & \bothmodels{2}{50}{orange!5} \\
					& Weight decay & \bothmodels{4}{1e-6 }{olive!5} \\
					& LR of weight & \bothmodels{2}{2e-1}{olive!5} & \bothmodels{2}{1e0}{orange!5} \\
					& LR of bias & \bothmodels{2}{4.8e-3}{olive!5} & \bothmodels{2}{2.4e-2}{orange!5} \\
					& Warmup epoch & \bothmodels{4}{10}{olive!5} \\
					& Training epoch & \bothmodels{2}{25}{olive!5} & \bothmodels{2}{50}{orange!5} \\
					\midrule
					\midrule
					& Hyperparam. & \bothmodels{2}{AS balanced}{white}  &  \bothmodels{2}{AS unbalanced}{white}\\
					\midrule
					& Optimizer & \bothmodels{4}{Adam~\citep{Adam}}{olive!5} \\
					& Batch size & \bothmodels{2}{12}{white} & \bothmodels{2}{128}{white} \\
					& Weight decay & \bothmodels{4}{1e-7}{olive!5} \\
					& Learning rate & \bothmodels{4}{5e-5}{olive!5} \\
					& Warmup step & \bothmodels{4}{1000}{olive!5} \\
					& Training epoch & \bothmodels{2}{25}{white} & \bothmodels{2}{5}{white} \\
					& LR scheduler & \bothmodels{4}{MultiStepLR ($\gamma = 0.5$) }{olive!5} \\
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:optimizer_setups}
	Hyperparameters of the optimizers used for VA pre-training, AL fine-tuning, ESC50 classification, US8K classification, balanced AS classification, and unbalanced AS classification.
	The learning rate (LR) in balanced AS is scheduled by epoch: 5, 9, 10, 11, 12 epochs. In unbalanced AS it is scheduled by optimization step: 7.5, 15, 20, 25, 35, 40, 45, 50 thousand steps.
	}
\end{table}

==> table/novel_pivotable_audio_category.tex <==
\begin{table}[h]\small
	\centering
	{\setlength{\tabcolsep}{0.em} %{.25em}
	\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
	\begin{tabular}{@{} m{0.2\linewidth} @{\hspace{0.25cm}} m{0.85\linewidth} @{} m{0.01\linewidth}}
%	Model & Novel Audio Ctegory	\\
	\midrule
	+AT w/ GC & {\color{orange}{'Bee, wasp, etc.'}}, 'Female speech, woman speaking', {\color{orange}{'Insect'}}, 'Narration, monologue', 'Vibration' \\
	\midrule
	+AT w/ RC & 'Female speech, woman speaking', 'Narration, monologue', 'Vibration' \\
	\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:categories_pivotable_audio}
		Comparing against \modelname, the two fine-tuned versions of \modelname find novel categories of audio clips in pivotable AT pairs.
	}
\end{table}

==> table/old/classification_merged_prompt_v2.tex <==
\begin{table}[!t]
	{\setlength{\tabcolsep}{.2em}
		\makebox[\linewidth]{\resizebox{.95\linewidth}{!}{%
				\begin{tabular}{
						@{} p{0.4cm}
						@{\hspace{0.05cm}} p{2.7cm} 
						@{\hspace{0.35cm}} p{1.65cm} 
						@{\hspace{0.25cm}} p{1.65cm} 
						@{\hspace{0.25cm}} p{1.55cm} 
						@{}
					}
					%		&  & \multicolumn{2}{c}{\hspace{-2mm}{\scriptsize EK100 (R@5; \%) }} \\
					&  Model & ESC50 & US8K & AS \\ \toprule
					\multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize }}} 
%					&  AST-S      & 88.7$_{\pm 0.7}$       &   & 31.4$^\star$ \\
%					&  AST-P      & 95.6$_{\pm 0.4}$       &   &  \\
%					\cmidrule{2-5}
%					&  Random & 55.5$_{\pm 4.1}$ & 71.7$_{\pm 5.2}$ & \leavevmode{\phantom{0}}6.1 \\
%					&  CLIP & 89.7$_{\pm 1.5}$ & 82.5$_{\pm 6.0}$ & 17.2 \\
					% 		&  \modelname probe & 79.3$_{\pm 3.0}$ & 82.0$_{\pm 4.7}$ & 18.1 \\
%					&  \modelname & \textbf{95.7}$_{\pm 1.4}$ & \textbf{86.0}$_{\pm 2.8}$ & \textbf{37.9} \\
					&  Supervised & \text{95.7}$_{\pm 1.4}$ & \text{86.0}$_{\pm 2.8}$ & \text{37.9} \\
					
					% 		& +AT w/ GC & \textbf{96.3}$_{\pm 0.6}$ & 81.0$_{\pm 5.14}$ & 37.9 \\ 
					\midrule
					% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/ $p$}}} 
					\cmidrule{2-5}
					\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot}}} 
					% 		&  CLIP      &  1.9   &  9.2 & 0.6 \\
					% 		\cmidrule{2-5}
					&  VA-Rand & 37.6{\footnotesize (33.0)} & 41.9{\footnotesize (38.1)} & \leavevmode{\phantom{0}}1.7{\footnotesize (\phantom{0}2.0)} \\
					&  \modelname     &   57.1{\footnotesize (49.9)}   & 44.7{\footnotesize (37.8)}  &  \leavevmode{\phantom{0}}2.6{\footnotesize (\phantom{0}2.8)} \\
					\cmidrule{2-5}
					&  +AT w/ GL     &   67.4{\footnotesize (64.3)}    &  62.9{\footnotesize (60.9)}   &  15.4{\footnotesize (\textbf{18.9})}  \\
					&  +AT w/ GC     &  69.2 {\footnotesize (64.3)}    &  \textbf{71.7}{\footnotesize (67.1)}  & 13.3{\footnotesize (13.6)} \\
					& AudioCLIP$^*$ (ZS) & \textbf{69.4} & 68.7 & -- \\
					\cdashlinelr{2-5}
					
	 		 		&  +AT w/ AC      &   62.8{\footnotesize (55.7)}   &  54.0{\footnotesize (47.0)}  &  11.6{\footnotesize (12.3)} \\
	 		 		&  +AT w/ FC     &  62.5{\footnotesize (58.0)}    & 52.7{\footnotesize (50.0)}   & 11.2{\footnotesize (12.2)} \\
	 		 		&  +AT w/ VC     &   61.9{\footnotesize (58.0)}   &  52.7{\footnotesize (50.3)}  &  \leavevmode{\phantom{0}}8.9{\footnotesize (10.7)} \\
	 		 		&  +AT w/ RC     &   51.6{\footnotesize (36.1)}    &  42.3{\footnotesize (28.5)}   &  \leavevmode{\phantom{0}}4.1{\footnotesize (\phantom{0}4.6)} \\
	 		 		& Wav2CLIP (ZS) & 41.4 & 40.4 & -- \\
					% 		\midrule
					% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/o $p$}}} 
					% 		&  CLIP      &   2.2   &  6.1  &  0.6 \\
					% 		\cmidrule{2-5}
					%         &  VA-Rand     & 33.0 & 38.1 & \leavevmode{\phantom{0}}2.0 \\
					% 		&  \modelname     &   49.9  &  37.8  &  \leavevmode{\phantom{0}}2.8 \\
					% 		\cmidrule{2-5}
%					 		&  +AT w/ VC     &   58.0   &  50.3  &  10.7 \\
%					 		&  +AT w/ AC      &  55.7   &  47.0  &  12.3 \\
%					 		&  +AT w/ FC     &  58.0    & 50.0   & 12.2 \\
%					 		&  +AT w/ GC     &   64.3   &  67.1  &  13.6 \\
%					 		&  +AT w/ RC     &   36.1   &  28.5  &  \leavevmode{\phantom{0}}4.6 \\
%					 		&  +AT w/ GL     &   64.3   &  60.9  &  18.9 \\
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:zeroshot-clf-merged-prompt}
		Zero-shot audio classification accuracies (\%) on ESC50 and US8K and mAPs (\%) on AS. 
%		AST-S and AST-P are the state-of-the-art models from~\citet{AST}.
		% 		$^\star$ indicates that we follow AST's settings and train and evaluate it on our data.
%		In the supervised setting, Random, CLIP, \modelname, and "+AT w/ GC" indicate that the audio encoder is initialized randomly, from CLIP, and from \modelname, respectively.
		"Supervised" indicates that we fine-tune \modelname for supervised audio classification. 
		% from \modelname, and from \modelname+AT (fine-tuned on gold AT pairs of AudioCaps), respectively.
		In the zero-shot setting, we use a prompt `\textit{the sound of}' by default; accuracies in the parenthesis are obtained without using the prompt. "+AT" means that we fine-tune \modelname on AT pairs curated through different ways.
		% 		$p$ represents the prompt `the sound of'. VC, AC, FC, RC, GC indicate different caption augmentation strategies (see Section~\ref{sec:audio_text_aug} for details).
		% 		and stand for \textbf{V}ision-focused, \textbf{A}udio-focused, \textbf{F}ree (generated by GPT-J), \textbf{G}old captions, and \textbf{R}andom gold captions, respectively. GL means that \textbf{G}old \textbf{L}abels of audios are used as captions.
	}
\end{table}

==> table/retrieval.tex <==
\begin{table*}[!t]\small
	\centering
	{\setlength{\tabcolsep}{1.2em} %{.25em}
		\makebox[\linewidth]{\resizebox{1.\linewidth}{!}{%
				\begin{tabular}{l@{} p{2.5cm} rrrrrrrr}
					\toprule
					& \multirow{3}{*}{Model} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
					\cmidrule{3-10}
					& & \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text} &  \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text}\\ 
					%	\cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8}
					& & {\scriptsize R$@$1} & {\scriptsize R$@$10} & 
					{\scriptsize R$@$1} & {\scriptsize R$@$10} &   
					{\scriptsize R$@$1} & {\scriptsize R$@$10} & 
					{\scriptsize R$@$1} & {\scriptsize R$@$10}\\ 
					\midrule
%					& \citet{audio_retrieval} & $18.0_{\pm0.2}$&$62.0_{\pm0.5}$&$ 21.0_{\pm0.8} $&$62.7_{\pm1.6}$ & $4.0_{\pm0.2}$&$25.4_{\pm0.5}$&$ 4.8_{\pm0.4} $&$25.8_{\pm1.7}$ \\
					& Supervised SOTA & $18.0$&$62.0$&$ 21.0$&$62.7$ & $4.0$&$25.4$&$ 4.8 $&$25.8$ \\
				% 	& CLIP & 0.0 & 1.3 & 0.2 & 2.0  &  0.1 & 1.3 & 0.2 & 1.0 \\
					& VA-Rand & 1.3 & 7.3 & 5.6 & 24.5 & 1.3 & 7.5 & 3.2 & 13.5 \\
					& \modelname & 0.8 & 7.9 & 10.1 & 38.1 & 1.9 & 9.5 & 7.0 & 25.6\\
					\midrule
					&  +AT w/ GL     & 12.4 & 52.9 & 13.0 & 51.2 & 6.7 & 29.0 & 6.8 & 27.0 \\
					&  +AT w/ GC     & \textbf{27.7} & \textbf{78.0} & \textbf{34.3} & \textbf{79.7} & \textbf{11.1} & \textbf{40.5} & \textbf{11.8} & \textbf{41.0}  \\
					\cdashlinelr{0-9}
					&  +AT w/ AC     & 9.9 & 45.6 & 15.2 & 52.9  & 6.7 & 29.1 & 7.1 & 30.7\\
					&  +AT w/ FC     & 8.9 & 41.5 & 14.7 & 50.0   & 6.5 & 27.7 & 7.8 & 29.7 \\
					&  +AT w/ VC     & 6.9 & 35.7 & 13.5 & 49.4 & 5.5 & 25.6 & 7.6 & 28.2 \\
					&  +AT w/ RC     & 3.8 & 19.9 & 10.7 & 38.1 & 3.5 & 16.9 & 5.5 & 24.9 \\
					\midrule
					& OracleAV-CLIP & 4.8 & 27.8 & 6.6 & 31.2 &\phantom{.}&\phantom{.}&\phantom{.}&\phantom{.}\\
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:audiocap-retrieval_test}
		Audio caption retrieval performance (\%) on AudioCaps test set and Clotho evaluation set. "Supervised SOTA" indicates the supervised state of the art from~\citet{audio_retrieval}. OracleAV-CLIP: we replace audio with the corresponding image and evaluate image-text retrieval performance of CLIP~\citep{CLIP}. For each Clotho audio clip, we extract an audio clip which has a duration of at most 18 seconds and up-sample the positional embeddings accordingly.
		VA-Rand and \modelname indicates that, in VA pre-training, the audio encoder is initialized randomly and from CLIP, respectively. We further fine-tune \modelname on AT data, which is curated using different ways: GL, GC, AC, FC, VC, and RC (see Table~\ref{tab:al_curation} for details).
% 		\jack{I think this table could be merged with the classification one next to it.} \yanpeng{I reverted because the merged looks too small and crowded.}
	}
	\vspace{-.15em}
\end{table*}
% 	\vspace{0.45cm}
% \begin{table*}[!t]\small
% 	\centering
% 	{\setlength{\tabcolsep}{0.em} %{.25em}
% 		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
% 				\begin{tabular}{@{} m{0.1\linewidth} @{\hspace{0.05cm}} m{0.75\linewidth} @{}}
% 					\toprule
% 					\textbf{GL} & \textbf{G}old textual \textbf{L}abels of audio clips are used to construct AT pairs. \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{Gurgling}}\\
% 					\midrule
% 					\textbf{GC} & \textbf{G}old \textbf{C}aptions from AudioCaps provide an upper bound on the quality of AT alignment. \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{Children screaming in the background as the sound of water flowing by.}} \\
% 					\midrule
% 					\textbf{AC}  & \textbf{A}udio-focused \textbf{C}aptions originate from the training captions of AudioCaps and Clotho. We perform caption retrieval by using CLIP and the prompt "the sound of". \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{A balloon is rubbed quickly and slowly to make squeaking sounds.}} \\
% 					\midrule
% 					\textbf{FC} & \textbf{F}ree \textbf{C}aptions are generated by priming GPT-J with MSCOCO captions. We perform caption retrieval by using CLIP and the prompt "a photo of". \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{The blue colored person is jumping on the white and yellow beach ball.}} \\					
% 					\midrule
% 					\textbf{VC} & \textbf{V}ision-focused \textbf{C}aptions originate from MSCOCO. We perform caption retrieval by using CLIP and the prompt "a photo of". \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{A sky view looking at a large parachute in the sky.}}\\
% 					\midrule
% 					\textbf{RC} & \textbf{R}andom \textbf{C}aptions indicates that we break the gold AT alignment in AudioCaps by randomly sampling a caption for each audio clip. They are used as a lower bound on the quality of AT alignment. \\
% 				% 	\cmidrule{2-2}
% 					example & \coloredrow{1}{olive!5}{\textit{A whoosh sound is heard loudly as a car revs its engines.}} \\
% 					\bottomrule
% 	\end{tabular}}}}
% 	\caption{\label{tab:al_curation}
% 		Different ways of curating AT pairs. \textit{Gurgling} is described as "the bubbling sound of water flowing through a narrow constriction, such as from a bottle with a narrow neck". The example comes from this YouTube video: \href{https://www.youtube.com/watch?v=1O7-QuhweZE}{1O7-QuhweZE}. The video clip starts at 19 seconds and lasts for 10 seconds (see video frames used for caption retrieval in Figure~\ref{fig:example_vframes}).
% 		%\youngjae{How about getting these two tables close to each other like this? and make the table3 simple. can I give very small frame lapse for the video?}
% 	}
% \end{table*}

% \begin{table*}[t!]\small
% \centering
% {\setlength{\tabcolsep}{.25em}
% \makebox[\linewidth]{\resizebox{\linewidth}{!}{%
% \begin{tabular}{llccccccccc}
% 	\toprule
% 	& \multirow{3}{*}{Model} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
% 	\cmidrule{3-10}
% 	& & \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text} &  \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text}\\ 
% %	\cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8}
% 	& & {\scriptsize R$@$1} & {\scriptsize R$@$10} & 
% 	{\scriptsize R$@$1} & {\scriptsize R$@$10} &   
% 	{\scriptsize R$@$1} & {\scriptsize R$@$10} & 
% 	{\scriptsize R$@$1} & {\scriptsize R$@$10} & \\ 
% 	\midrule
% 	& \citet{audio_retrieval} & $4.0_{\pm0.2}$&$25.4_{\pm0.5}$&$ 4.8_{\pm0.4} $&$25.8_{\pm1.7}$& $4.0_{\pm0.2}$&$25.4_{\pm0.5}$&$ 4.8_{\pm0.4} $&$25.8_{\pm1.7}$ \\
% 	& CLIP & \phantom{0}0.2 & \phantom{0}2.6 & \phantom{0}0.2 & \phantom{0}1.8 &      \phantom{0}0.0 & \phantom{0}0.9 & \phantom{0}0.2 & \phantom{0}1.0 \\
% 	\midrule
% 	& VA & \phantom{0}1.5 & \phantom{0}8.4 & 10.2 & 46.7 &    \phantom{0}1.6 & \phantom{0}9.2 & \phantom{0}6.5 & 29.7 \\
% 	&  +AT w/ VC     &   \phantom{0}8.4 & 42.2 & 17.7 & 58.0 &     \phantom{0}5.3 & 26.0 & \phantom{0}7.0 & 29.6\\
% 	&  +AT w/ AC      &  10.6 & 52.3 & 19.5 & 58.7 &   \phantom{0}6.2 & 29.0 & \phantom{0}7.2 & 31.2\\
% 	&  +AT w/ FC     &      &    &  \\
% 	&  +AT w/ GC     &   33.6 & 84.3 & 42.0 & 86.6 &   10.1 & 41.8 & 12.1 & 40.8\\
% 	&  +AT w/ RC     &   \phantom{0}5.0 & 26.8 & 11.6 & 47.4 &   \phantom{0}3.1 & 16.5 & \phantom{0}5.7 & 24.7\\
% 	&  +AT w/ GL     &  16.3 & 62.7 & 19.7 & 62.1&   \phantom{0}6.0 & 28.6 & \phantom{0}6.1 & 28.4 \\
% 	\bottomrule
% \end{tabular}}}}
% 	\caption{\label{tab:audiocap-retrieval}
% 	Audio caption retrieval performance on AudioCaps and Clotho validation sets.
% }
% \end{table*}

==> table/retrieval_and_zero_shot_clf_in_one.tex <==

\begin{figure*}[ht!]
   \begin{minipage}{.63\linewidth}
   \resizebox{\linewidth}{!}{
      \begin{tabular}{l@{}p{3cm} rrrrrrrr}
					\toprule
					& \multirow{3}{*}{Model} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
					\cmidrule{3-10}
					& & \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text} &  \multicolumn{2}{c}{Text$\rightarrow$Audio} & \multicolumn{2}{c}{Audio$\rightarrow$Text}\\ 
					%	\cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8}
					& & {\scriptsize R$@$1} & {\scriptsize R$@$10} & 
					{\scriptsize R$@$1} & {\scriptsize R$@$10} &   
					{\scriptsize R$@$1} & {\scriptsize R$@$10} & 
					{\scriptsize R$@$1} & {\scriptsize R$@$10}\\ 
					\midrule
%					& \citet{audio_retrieval} & $18.0_{\pm0.2}$&$62.0_{\pm0.5}$&$ 21.0_{\pm0.8} $&$62.7_{\pm1.6}$ & $4.0_{\pm0.2}$&$25.4_{\pm0.5}$&$ 4.8_{\pm0.4} $&$25.8_{\pm1.7}$ \\
					& \citet{audio_retrieval} & $18.0$&$62.0$&$ 21.0$&$62.7$ & $4.0$&$25.4$&$ 4.8 $&$25.8$ \\
				% 	& CLIP & 0.0 & 1.3 & 0.2 & 2.0  &  0.1 & 1.3 & 0.2 & 1.0 \\
					& VA-Rand & 1.3 & 7.3 & 5.6 & 24.5 & 1.3 & 7.5 & 3.2 & 13.5 \\
					& \modelname & 0.8 & 7.9 & 10.1 & 38.1 & 1.9 & 9.5 & 7.0 & 25.6\\
					\toprule
					& CLIP$^\dagger$ & 4.8 & 27.8 & 6.6 & 31.2 \\
					\toprule
					&  +AT w/ GL     & 12.4 & 52.9 & 13.0 & 51.2 & 6.7 & 29.0 & 6.8 & 27.0 \\
					&  +AT w/ GC     & \textbf{27.7} & \textbf{78.0} & \textbf{34.3} & \textbf{79.7} & \textbf{11.1} & \textbf{40.5} & \textbf{11.8} & \textbf{41.0}  \\					
					&  +AT w/ AC     & 9.9 & 45.6 & 15.2 & 52.9  & 6.7 & 29.1 & 7.1 & 30.7\\
					&  +AT w/ FC     & 8.9 & 41.5 & 14.7 & 50.0   & 6.5 & 27.7 & 7.8 & 29.7 \\
					&  +AT w/ VC     & 6.9 & 35.7 & 13.5 & 49.4 & 5.5 & 25.6 & 7.6 & 28.2 \\
					&  +AT w/ RC     & 3.8 & 19.9 & 10.7 & 38.1 & 3.5 & 16.9 & 5.5 & 24.9 \\
					\bottomrule
	\end{tabular}
    }
    \captionof{table}{
		Audio caption retrieval performance (\%) on AudioCaps test set and Clotho evaluation set. $^\dagger$ indicates that we replace audio with the corresponding image and evaluate image-text retrieval performance of CLIP~\citep{CLIP}. For each Clotho audio clip, we extract an audio clip which has a duration of at most 18 seconds and upsample the position embeddings accordingly.
		VA-Rand and \modelname indicates that, in VA pre-training, the audio encoder is initialized randomly and from CLIP, respectively. We further fine-tune \modelname on AT data, which is curated using different ways: VC, AC, FC, GC, RC, and GL (see Table~\ref{tab:al_curation} for details). \jack{I think this table could be merged with the classification one next to it.}
	}
	\label{tab:audiocap-retrieval_test}
    \end{minipage}
    %\hfill
    \begin{minipage}{.35\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
	\begin{tabular}{
			@{} p{0.4cm} 
			@{\hspace{0.05cm}} p{2.cm} 
			@{\hspace{0.35cm}} p{1.65cm} 
			@{\hspace{0.25cm}} p{1.65cm} 
			@{\hspace{0.25cm}} p{1.55cm} 
			@{}
	}
%		&  & \multicolumn{2}{c}{\hspace{-2mm}{\scriptsize EK100 (R@5; \%) }} \\
		&  Model & ESC50 & US8K & AS \\ \toprule
		\multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize }}} 
% 		&  AST-S      & 88.7$_{\pm 0.7}$       &   & 31.4$^\star$ \\
% 		&  AST-P      & 95.6$_{\pm 0.4}$       &   &  \\
% 		\cmidrule{2-5}
% 		&  Random & 55.5$_{\pm 4.1}$ & 71.7$_{\pm 5.2}$ & \leavevmode{\phantom{0}}6.1 \\
% 		&  CLIP & 89.7$_{\pm 1.5}$ & 82.5$_{\pm 6.0}$ & 17.2 \\
% 		&  \modelname probe & 79.3$_{\pm 3.0}$ & 82.0$_{\pm 4.7}$ & 18.1 \\
		&  Supervised & \textbf{95.7}$_{\pm 1.4}$ & \textbf{86.0}$_{\pm 2.8}$ & \textbf{37.9} \\
% 		& +AT w/ GC & \textbf{96.3}$_{\pm 0.6}$ & 81.0$_{\pm 5.14}$ & 37.9 \\ 
		\midrule
% 		\multirow{8}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot w/ $p$}}} 
		\multirow{3}{*}{\rotatebox[origin=c]{90}{{\footnotesize Zero-shot}}} 
% 		&  CLIP      &  1.9   &  9.2 & 0.6 \\
% 		\cmidrule{2-5}
        &  VA-Rand & 37.6{\footnotesize (33.0)} & 41.9{\footnotesize (38.1)} & \leavevmode{\phantom{0}}1.7{\footnotesize (\phantom{0}2.0)} \\
		&  \modelname     &   57.1{\footnotesize (49.9)}   & 44.7{\footnotesize (37.8)}  &  \leavevmode{\phantom{0}}2.6{\footnotesize (\phantom{0}2.8)} \\
		\cmidrule{2-5}
		&  +AT w/ GC     &  51.6{\footnotesize (36.1)}    &  42.3{\footnotesize (28.5)}  & \phantom{0}4.1{\footnotesize (\phantom{0}4.6)} \\
		&  +AT w/ GC     &  69.2{\footnotesize (64.3)}    &  71.7{\footnotesize (67.1)}  & 13.3{\footnotesize (13.6)} \\
		\bottomrule
	\end{tabular}}
	\captionof{table}{
		Supervised and zero-shot audio classification accuracies (\%) on ESC50 and US8K and mAPs (\%) on AS. 
		AST-S and AST-P are the state-of-the-art models from~\citet{AST}.
% 		$^\star$ indicates that we follow AST's settings and train and evaluate it on our data.
        In the supervised setting, Random, CLIP, \modelname, and "+AT w/ GC" indicate that the audio encoder is initialized randomly, from CLIP, and from \modelname, respectively.
        % from \modelname, and from \modelname+AT (fine-tuned on gold AT pairs of AudioCaps), respectively.
        In the zero-shot setting, we use a prompt "the sound of" by default; accuracies in the parenthesis are obtained without using the prompt. "+AT w/ GC" means that we fine-tune \modelname on gold AT pairs of AudioCaps.
% 		$p$ represents the prompt `the sound of'. VC, AC, FC, RC, GC indicate different caption augmentation strategies (see Section~\ref{sec:audio_text_aug} for details).
% 		and stand for \textbf{V}ision-focused, \textbf{A}udio-focused, \textbf{F}ree (generated by GPT-J), \textbf{G}old captions, and \textbf{R}andom gold captions, respectively. GL means that \textbf{G}old \textbf{L}abels of audios are used as captions.
	\jack{I think this table could be merged with the retrieval one next to it.}}
	\label{tab:zeroshot-clf}
	\label{tab:ek100table}
    \end{minipage}
\end{figure*}
